XBound-Former: Toward Cross-scale Boundary Modeling in Transformers

Skin lesion segmentation from dermoscopy images is of great significance in the quantitative analysis of skin cancers, which is yet challenging even for dermatologists due to the inherent issues, i.e., considerable size, shape and color variation, and ambiguous boundaries. Recent vision transformers have shown promising performance in handling the variation through global context modeling. Still, they have not thoroughly solved the problem of ambiguous boundaries as they ignore the complementary usage of the boundary knowledge and global contexts. In this paper, we propose a novel cross-scale boundary-aware transformer, \textbf{XBound-Former}, to simultaneously address the variation and boundary problems of skin lesion segmentation. XBound-Former is a purely attention-based network and catches boundary knowledge via three specially designed learners. We evaluate the model on two skin lesion datasets, ISIC-2016\&PH$^2$ and ISIC-2018, where our model consistently outperforms other convolution- and transformer-based models, especially on the boundary-wise metrics. We extensively verify the generalization ability of polyp lesion segmentation that has similar characteristics, and our model can also yield significant improvement compared to the latest models.

==> figures/FigureAblation.tex <==
 \begin{figure}[t]
    \center{\includegraphics[width=\linewidth]{images/Ablation Experiment Comparison.pdf}}
    \caption{Visual comparison of ablation experiments on skin lesion segmentation. The areas indicated by the red arrow demonstrate that the segmentation of our method here has been significantly improved.
    }
    \label{fig:ablation}
\end{figure}

==> tables/Table_AblationResult.tex <==
\begin{table*}[ht]
    \caption{Quantitative comparison of different components of our proposed method on ISIC-2018 dataset. ``Trans" and ``BAG" mean Transformer module and Boundary-wise Attention Gate module are added on the basis of Baseline. ``Cross" indicates that cross attention was implemented between dual path Transformer in the Dual Path BAT network. ``Enc" and ``Dec" refer to BAG was used after Transformer Encoder and Decoder. Values in the subscript denote the improvement compared to the Baseline.}\label{exp}
\centering
\renewcommand\arraystretch{1.2}
\setlength\tabcolsep{4pt}
\begin{tabular}{cccccccccc}
\hline
Method & Trans & BAG & Cross & Params(M) & FLOPs(G) & IoU(\%)$\uparrow$ & Dice(\%)$\uparrow$ & ASSD(pix)$\downarrow$ & HD95(pix)$\downarrow$\\
\hline
Baseline(DeepLabV3) & & &  & 39.0 & 47.9 & 83.27 & 89.99 & 1.53 & 8.96\\
Transformer & \checkmark & & & 40.3 & 48.9 & $87.13_{+3.86}$ & $92.64_{+2.65}$ & $0.71_{-0.82}$ & $4.48_{-4.48}$\\
BAT(Enc) & \checkmark & \checkmark & & 40.6 & 49.2 & $87.82_{+4.55}$ & $93.09_{+3.10}$ & $0.76_{-0.77}$ & $4.48_{-4.48}$\\
BAT(Dec) & \checkmark & \checkmark & & 40.6 & 49.3 & $87.93_{+4.66}$ & $93.20_{+3.21}$ & $0.71_{-0.82}$ & $4.46_{-4.50}$\\
BAT(Enc+Dec) & \checkmark & \checkmark & & 40.9 & 49.6 & $88.00_{+4.73}$ & $93.24_{+3.25}$ & $0.67_{-0.86}$ & $4.12_{-4.84}$\\
Cross-BAT & \checkmark & \checkmark & \checkmark & 56.2 & 55.2 & $\bf{88.58_{+5.31}}$ & $\bf{93.60_{+3.61}}$ & $\bf{0.60_{-0.93}}$ & $\bf{3.63_{-5.33}}$\\
\hline
\end{tabular}
\label{tab:ablation}
\end{table*}
